An Evaluation of Real-time Adaptive Sampling Change Point Detection Algorithm using KCUSUM

Detecting abrupt changes in real-time data streams from scientific simulations presents a challenging task, demanding the deployment of accurate and efficient algorithms. Identifying change points in live data stream involves continuous scrutiny of incoming observations for deviations in their statistical characteristics, particularly in high-volume data scenarios. Maintaining a balance between sudden change detection and minimizing false alarms is vital. Many existing algorithms for this purpose rely on known probability distributions, limiting their feasibility. In this study, we introduce the Kernel-based Cumulative Sum (KCUSUM) algorithm, a non-parametric extension of the traditional Cumulative Sum (CUSUM) method, which has gained prominence for its efficacy in online change point detection under less restrictive conditions. KCUSUM splits itself by comparing incoming samples directly with reference samples and computes a statistic grounded in the Maximum Mean Discrepancy (MMD) non-parametric framework. This approach extends KCUSUM's pertinence to scenarios where only reference samples are available, such as atomic trajectories of proteins in vacuum, facilitating the detection of deviations from the reference sample without prior knowledge of the data's underlying distribution. Furthermore, by harnessing MMD's inherent random-walk structure, we can theoretically analyze KCUSUM's performance across various use cases, including metrics like expected delay and mean runtime to false alarms. Finally, we discuss real-world use cases from scientific simulations such as NWChem CODAR and protein folding data, demonstrating KCUSUM's practical effectiveness in online change point detection.

==> refer.tex <==
@article{Lorden71,
author = {G. Lorden},
title = {{Procedures for Reacting to a Change in Distribution}},
volume = {42},
journal = {The Annals of Mathematical Statistics},
number = {6},
publisher = {Institute of Mathematical Statistics},
pages = {1897 -- 1908},
year = {1971},
doi = {10.1214/aoms/1177693055},
URL = {https://doi.org/10.1214/aoms/1177693055}
}
@article{Lorden70,
author = {Gary Lorden},
title = {{On Excess Over the Boundary}},
volume = {41},
journal = {The Annals of Mathematical Statistics},
number = {2},
publisher = {Institute of Mathematical Statistics},
pages = {520 -- 527},
year = {1970},
doi = {10.1214/aoms/1177697092},
URL = {https://doi.org/10.1214/aoms/1177697092}
}
@article{Muandet07,
  langid = {english},
  title = {Kernel {{Mean Embedding}} of {{Distributions}}: {{A Review}} and {{Beyond}}},
  volume = {10},
  issn = {1935-8237, 1935-8245},
  url = {https://www.nowpublishers.com/article/Details/MAL-060},
  doi = {10.1561/2200000060},
  shorttitle = {Kernel {{Mean Embedding}} of {{Distributions}}},
  abstract = {Kernel Mean Embedding of Distributions: A Review and Beyond},
  number = {1-2},
  journaltitle = {Foundations and Trends® in Machine Learning},
  shortjournal = {MAL},
  urldate = {2018-08-30},
  date = {2017-06-28},
  pages = {1-141},
  author = {Muandet, Krikamol and Fukumizu, Kenji and Sriperumbudur, Bharath and Schölkopf, Bernhard},
  file = {/home/dimitri/Nextcloud/Zotero/storage/3A6PW3II/Muandet et al. - 2017 - Kernel Mean Embedding of Distributions A Review a.pdf;/home/dimitri/Nextcloud/Zotero/storage/7DS27M8D/MAL-060.html}
}

@book{Basseville93,
  TITLE = {{Detection of Abrupt Changes - Theory and Application}},
  AUTHOR = {Basseville, Mich{\`e}le and Nikiforov, Igor V.},
  URL = {https://hal.science/hal-00008518},
  PUBLISHER = {{Prentice Hall, Inc. - http://people.irisa.fr/Michele.Basseville/kniga/}},
  PAGES = {550},
  YEAR = {1993},

}

@book{Gallager95,
  title={Discrete Stochastic Processes},
  author={Gallager, R.G.},
  isbn={9780792395836},
  lccn={95014891},
  series={The Springer International Series in Engineering and Computer Science},
  url={https://books.google.com/books?id=jhffF8WWNLkC},
  year={1995},
  publisher={Springer US}
}
@article{Moustakides09,
   title={Numerical Comparison of CUSUM and Shiryaev–Roberts Procedures for Detecting Changes in Distributions},
   volume={38},
   ISSN={1532-415X},
   url={http://dx.doi.org/10.1080/03610920902947774},
   DOI={10.1080/03610920902947774},
   number={16–17},
   journal={Communications in Statistics - Theory and Methods},
   publisher={Informa UK Limited},
   author={Moustakides, George V. and Polunchenko, Aleksey S. and Tartakovsky, Alexander G.},
   year={2009},
   month=aug, pages={3225–3239} }
@book{Poor08,
title = "Quickest detection",
abstract = "The problem of detecting abrupt changes in the behavior of an observed signal or time series arises in a variety of fields, including climate modeling, finance, image analysis, and security. Quickest detection refers to real-time detection of such changes as quickly as possible after they occur. Using the framework of optimal stopping theory, this book describes the fundamentals underpinning the field, providing the background necessary to design, analyze, and understand quickest detection algorithms. For the first time the authors bring together results which were previously scattered across disparate disciplines, and provide a unified treatment of several different approaches to the quickest detection problem. This book is essential reading for anyone who wants to understand the basic statistical procedures for change detection from a fundamental viewpoint, and for those interested in theoretical questions of change detection. It is ideal for graduate students and researchers of engineering, statistics, economics, and finance.",
author = "Poor, {H. Vincent} and Olympia Hadjiliadis",
note = "Publisher Copyright: {\textcopyright} Cambridge University Press 2009.",
year = "2008",
month = jan,
day = "1",
doi = "10.1017/CBO9780511754678",
language = "English (US)",
isbn = "9780521621045",
volume = "9780521621045",
publisher = "Cambridge University Press",
address = "United Kingdom",
}
@article{Page54,
  title={CONTINUOUS INSPECTION SCHEMES},
  author={E. S. Page},
  journal={Biometrika},
  year={1954},
  volume={41},
  pages={100-115},
  url={https://api.semanticscholar.org/CorpusID:121530032}
}
@article{Feller48,
author = {W. Feller},
title = {{On the Kolmogorov-Smirnov Limit Theorems for Empirical Distributions}},
volume = {19},
journal = {The Annals of Mathematical Statistics},
number = {2},
publisher = {Institute of Mathematical Statistics},
pages = {177 -- 189},
year = {1948},
doi = {10.1214/aoms/1177730243},
URL = {https://doi.org/10.1214/aoms/1177730243}
}
@article{Anderson62,
  title={On the distribution of the two-sample Cramer-von Mises criterion},
  author={Anderson, Theodore W},
  journal={The Annals of Mathematical Statistics},
  pages={1148--1159},
  year={1962},
  publisher={JSTOR}
}
@article{Pettitt76,
  title={A two-sample Anderson-Darling rank statistic},
  author={Anthony N. Pettitt},
  journal={Biometrika},
  year={1976},
  volume={63},
  pages={161-168},
  url={https://api.semanticscholar.org/CorpusID:119481227}
}
@article{Gretton12,
  author  = {Arthur Gretton and Karsten M. Borgwardt and Malte J. Rasch and Bernhard Sch{{\"o}}lkopf and Alexander Smola},
  title   = {A Kernel Two-Sample Test},
  journal = {Journal of Machine Learning Research},
  year    = {2012},
  volume  = {13},
  number  = {25},
  pages   = {723-773},
  url     = {http://jmlr.org/papers/v13/gretton12a.html}
}
@article{Gartner03,
author = {Gärtner, Thomas},
year = {2003},
month = {07},
pages = {49-58},
title = {A Survey of Kernels for Structured Data},
volume = {5},
journal = {SIGKDD Explorations},
doi = {10.1145/959242.959248}
}

@misc{Vichy10,
      title={Graph Kernels}, 
      author={S. V. N. Vishwanathan and Karsten M. Borgwardt and Imre Risi Kondor and Nicol N. Schraudolph},
      year={2008},
      eprint={0807.0093},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}
@book{Shewhart31,
  title={Statistical Method from the Viewpoint of Quality Control},
  author={Shewhart, W.A. and Deming, W.E.},
  lccn={40004774},
  url={https://books.google.com/books?id=-VptAAAAMAAJ},
  year={1939},
  publisher={Graduate School, The Department of Agriculture}
}
@book{Wald47,
  title={Sequential analysis},
  author={Wald, A.},
  url={https://books.google.com/books?id=0nREAAAAIAAJ},
  year={1947},
  publisher={J. Wiley \& sons, Incorporated}
}
@inproceedings{Harchaoui09,
 author = {Harchaoui, Za\"{\i}d and Moulines, Eric and Bach, Francis},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {D. Koller and D. Schuurmans and Y. Bengio and L. Bottou},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {Kernel Change-point Analysis},
 url = {https://proceedings.neurips.cc/paper_files/paper/2008/file/08b255a5d42b89b0585260b6f2360bdd-Paper.pdf},
 volume = {21},
 year = {2008}
}
@book{Brodsky931,
  title={Nonparametric Methods in Change Point Problems},
  author={Brodsky, E. and Darkhovsky, B.S.},
  isbn={9789048142408},
  series={Mathematics and Its Applications},
  url={https://books.google.com/books?id=c5ADkgAACAAJ},
  year={2010},
  publisher={Springer Netherlands}
}
@inproceedings{Brodsky93,
  title={Nonparametric Methods in Change Point Problems},
  author={Boris Brodsky and Boris S. Darkhovsky},
  year={1993},
  url={https://api.semanticscholar.org/CorpusID:118958786}
}
@inproceedings{Li15,
  title={M-Statistic for Kernel Change-Point Detection},
  author={Shuang Li and Yao Xie and Hanjun Dai and Le Song},
  booktitle={Neural Information Processing Systems},
  year={2015},
  url={https://api.semanticscholar.org/CorpusID:5770615}
}
@article{Polunchenko10,
   title={On optimality of the Shiryaev–Roberts procedure for detecting a change in distribution},
   volume={38},
   ISSN={0090-5364},
   url={http://dx.doi.org/10.1214/09-AOS775},
   DOI={10.1214/09-aos775},
   number={6},
   journal={The Annals of Statistics},
   publisher={Institute of Mathematical Statistics},
   author={Polunchenko, Aleksey S. and Tartakovsky, Alexander G.},
   year={2010},
   month=dec }
@article{Haug22,
author = {Cheng-Der Fuh},
title = {{SPRT and CUSUM in hidden Markov models}},
volume = {31},
journal = {The Annals of Statistics},
number = {3},
publisher = {Institute of Mathematical Statistics},
pages = {942 -- 977},
keywords = {Brownian approximation, change point detection, CUSUM, First passage time, Products of random matrices, renewal theory, Wald's equation, Wald's identity},
year = {2003},
doi = {10.1214/aos/1056562468},
URL = {https://doi.org/10.1214/aos/1056562468}
}
@misc{Flynn19,
      title={Change Detection with the Kernel Cumulative Sum Algorithm}, 
      author={Thomas Flynn and Shinjae Yoo},
      year={2020},
      eprint={1903.01661},
      archivePrefix={arXiv},
      primaryClass={math.ST}
}
@article{Moustakides86,
author = {George V. Moustakides},
title = {{Optimal Stopping Times for Detecting Changes in Distributions}},
volume = {14},
journal = {The Annals of Statistics},
number = {4},
publisher = {Institute of Mathematical Statistics},
pages = {1379 -- 1387},
keywords = {62E, detection of changes, sequential analysis, stopping times},
year = {1986},
doi = {10.1214/aos/1176350164},
URL = {https://doi.org/10.1214/aos/1176350164}
}






